Simulating TeV gamma-ray morphologies of shell-type supernova remnants

Supernova remnant (SNR) shocks provide favourable sites of cosmic ray (CR) proton acceleration if the local magnetic field direction is quasi-parallel to the shock normal. Using the moving-mesh magneto-hydrodynamical (MHD) code AREPO we present a suite of SNR simulations with CR acceleration in the Sedov-Taylor phase that combine different magnetic field topologies, density distributions with gradients and large-scale fluctuations, and -- for our core-collapse SNRs -- a multi-phase interstellar medium with dense clumps with a contrast of $10^4$. Assuming the hadronic gamma-ray emission model for the TeV gamma-ray emission, we find that large-amplitude density fluctuations of $\delta\rho/\rho_0\gtrsim75$ per cent are required to strongly modulate the gamma-ray emissivity in a straw man's model in which the acceleration efficiency is independent of magnetic obliquity. However, this causes strong corrugations of the shock surface that are ruled out by gamma-ray observations. By contrast, magnetic obliquity-dependent acceleration can easily explain the observed variance in gamma-ray morphologies ranging from SN1006 (with a homogeneous magnetic field) to Vela Junior and RX J1713 (with a turbulent field) in a single model that derives from plasma particle-in-cell simulations. Our best-fit model for SN1006 has a large-scale density gradient of $ \nabla{n}\simeq 0.0034~\mathrm{cm}^{-3}~\mathrm{pc}^{-1} $ pointing from south-west to north-east and a magnetic inclination with the plane of the sky of $\lesssim10^\circ$. Our best-fit model for Vela Junior and RX J1713 adopts a combination of turbulent magnetic field and dense clumps to explain their TeV gamma-ray morphologies and moderate shock corrugations.

==> Makefile <==
# Makefile to produce the article.
PDFLATEX  =  TEXINPUTS=.//: BSTINPUTS=.//: pdflatex
LATEX  =  TEXINPUTS=.//: BSTINPUTS=.//: latex
DVIPS  =  dvips
FIGURES = 

.PRECIOUS: $(FIGURES)

default: ms.pdf

%.pdf :  $(FIGURES) %.tex
	$(PDFLATEX) $*.tex
	TEXINPUTS=:.// BSTINPUTS=:.// bibtex $*
	$(PDFLATEX) $*.tex
	$(PDFLATEX) $*.tex
	$(PDFLATEX) $*.tex
	make clean

%.ps :  $(FIGURES) %.tex
	$(LATEX) $*.tex
	TEXINPUTS=:.// BSTINPUTS=:.// bibtex $*
	$(LATEX) $*.tex
	$(LATEX) $*.tex
	$(LATEX) $*.tex
	$(DVIPS) -o $*.ps $*.dvi
	ps2pdf $*.ps
	make clean

figures/%.eps: figures/%_raw.eps figures/%.tex
	(cd figures; latex $*.tex; \
	dvips -E -o $*.eps $*.dvi; \
	perl -ane '{ s/%%BoundingBox: [-0-9]+/%%BoundingBox: 135/g; print}' $*.eps > tmp.eps; \
	mv tmp.eps $*.eps; \
	rm -f *.dvi *.log *.aux)

clean:
	rm -f *.log *.toc *.aux *.dvi *.bak *.blg *.obj *.out

realclean:
	rm -f *.log *.toc *.aux *.dvi *.obj *.bak *.bbl *.blg *.brf \
              *.pdf *.ps */*.ps *~ */*~ *.bak */*.bak 









